Surrogate uncertainty estimation for your time series forecasting black-box: learn when to trust

Machine learning models play a vital role in time series forecasting. These models, however, often overlook an important element: point uncertainty estimates. Incorporating these estimates is crucial for effective risk management, informed model selection, and decision-making.To address this issue, our research introduces a method for uncertainty estimation. We employ a surrogate Gaussian process regression model. It enhances any base regression model with reasonable uncertainty estimates. This approach stands out for its computational efficiency. It only necessitates training one supplementary surrogate and avoids any data-specific assumptions. Furthermore, this method for work requires only the presence of the base model as a black box and its respective training data. The effectiveness of our approach is supported by experimental results. Using various time-series forecasting data, we found that our surrogate model-based technique delivers significantly more accurate confidence intervals. These techniques outperform both bootstrap-based and built-in methods in a medium-data regime. This superiority holds across a range of base model types, including a linear regression, ARIMA, gradient boosting and a neural network.

==> tex/commented_experiments.tex <==
% \begin{table}
% \scriptsize
% \caption{Ranks of calibration metrics of all best models aggregated over Forecasting data. Best results are highlighted with \textbf{{bold}} font, second best results are \underline{{underscored}}
% }
% \label{tab:rank_all_best}
% \begin{adjustbox}{width=0.5\textwidth}
% \begin{tabular}{ccccc}
% \toprule
% \begin{tabular}{c}
% Model
% \end{tabular}&
% \begin{tabular}{c}
% RMSE
% \end{tabular}&
% \begin{tabular}{c}
% Miscal.\\
% Area
% \end{tabular}&
% \begin{tabular}{c}
% RMSCE
% \end{tabular}&
% \begin{tabular}{c}
% ENCE
% \end{tabular}\\
% \midrule
% OLS &  6.438 &  8.688 &  8.662 &  9.725 \\
% Surr ind. OLS &  6.438 & \textbf{4.462} & \textbf{4.45} & \textbf{4.125} \\
% Surr ind. OLS RBF kernel &  6.438 &  5.675 &  5.638 &  6.162 \\
% Surr I OLS &  6.438 & \underline{5.038} & \underline{4.938} & \underline{4.688} \\
% Surr II OLS &  6.438 &  6.738 &  6.688 &  6.712 \\
% Surr III OLS &  6.438 &  7.338 &  7.462 &  7.15 \\
% Surr IV OLS &  6.438 &  6.388 &  6.462 &  5.275 \\
% GPR &  6.762 &  5.738 &  5.788 &  5.15 \\
% BSAP BS OLS & \textbf{5.15} &  8.137 &  8.25 &  10.8 \\
% Naive BS OLS &  7.55 &  8.137 &  8.2 &  8.875 \\
% ARIMA &  11.75 &  10.538 &  10.538 &  7.862 \\
% BSAP BS ARIMA & \underline{6.312} &  7.238 &  7.1 &  7.325 \\
% Naive BS ARIMA &  8.412 &  6.888 &  6.825 &  7.15 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/ARIMA_surr_cd-diagram_Miscalibration_Area.pdf}
%     \caption{ARIMA base surrogate model comparison of Miscal. Area on Forecasting data}
%     \label{fig:surr_cd_arima_miscal}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/CatBoost_surr_cd-diagram_Miscalibration_Area.pdf}
%     \caption{CatBoost base surrogate model comparison of Miscal. Area on Forecasting data}
%     \label{fig:surr_cd_catboost_miscal}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/c_change_ence.pdf}
%     \caption{Dependence of the surrogate uncertainty estimate quality metric ENCE on the hyperparameter $C$ for different number of generated points}
%     \label{fig:vary_c_ence}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/frac_change.pdf}
%     \caption{Dependence of the surrogate uncertainty estimate quality on the hyperparameter $frac$}
%     \label{fig:vary_frac}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/loans_short_base_models_results_AB.pdf}
%     \caption{Performance of base models on different train/test splits of Dataset A. Bigger horizon means bigger test size}
%     \label{fig:c_change}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/mortgages_short_base_models_results_AB.pdf}
%     \caption{Performance of base models on different train/test splits of Dataset A. Bigger horizon means bigger test size}
%     \label{fig:c_change}
% \end{figure}

